A Bio-inspired Asymmetric Double-Gate Ferroelectric FET for Emulating Astrocyte and Dendrite Dynamics in Neuromorphic Systems

Neuromorphic systems seek to replicate the functionalities of biological neural networks to attain significant improvements in performance and efficiency of AI computing platforms. However, these systems have generally remained limited to emulation of simple neurons and synapses; and ignored higher order functionalities enabled by other components of the brain like astrocytes and dendrites. In this work, drawing inspiration from biology, we introduce a compact Double-Gate Ferroelectric Field Effect Transistor (DG-FeFET) cell that can emulate the dynamics of both astrocytes and dendrites within neuromorphic architectures. We demonstrate that with a ferroelectric top gate for synaptic weight programming as in conventional synapses and a non-ferroelectric back gate, the DG-FeFET realizes a synapse with a dynamic gain modulation mechanism. This can be leveraged as an analog for a compact astrocyte-tripartite synapse, as well as enabling dendrite-like gain modulation operations. By employing a fully-depleted silicon-on-insulator (FDSOI) FeFET as our double-gate device, we validate the linear control of the synaptic weight via the back gate terminal (i.e., the gate underneath the buried oxide (BOX) layer) through comprehensive theoretical and experimental studies. We showcase the promise such a tripartite synaptic device holds for numerous important neuromorphic applications, including autonomous self-repair of faulty neuromorphic hardware mediated by astrocytic functionality. Coordinate transformations based on dragonfly prey-interception circuitry models are also demonstrated based on dendritic function emulation by the device. This work paves the way forward for developing truly "brain-like" neuromorphic hardware that go beyond the current dogma focusing only on neurons and synapses.

==> sections/Conclusion.tex <==
\section*{\large Conclusion}

In this work, we exploit a DG FeFET to implement a compact astrocyte tripartite synapse, whose hardware implementation has been recognized but remains long elusive. We theoretically and experimentally established the linear dependence of synaptic weight on the astrocyte, i.e., BG. Through combined device-to-algorithm co-design, we demonstrate interesting applications, including self-repair and homeostasis, that are enabled by the DG FeFET. These results show that DG FeFET, as an efficient hardware implementation of the astrocyte tripartite synapse, can augment existing neuromorphic hardware with new functionalities.

==> sections/Evaluation.tex <==
\section*{\textcolor{sared}{\large Application of astrocyte tripartite synapse}}

Next we evaluate the capability of DG-FeFET array in performing multiply-accumulation operation. Fig.\ref{fig:application}(a) shows a 7$\times$8 array that is used for demonstration. The column current is measured when activating different number of cells in that array. Fig.\ref{fig:application}(b) shows the swept current as a function of top gate bias for all the drain lines (i.e., 8 lines) in the array. With the read bias at 2V, the column current shows a linear trend with the number of activated cells, as shown in Fig.\ref{fig:application}(c). With the crossbar macro introduced in Fig.\ref{fig:introduction}(c), several SNN applications of the astrocyte tripartite synapses are considered.
First, the self-repair function is studied, which has been introduced in Fig.\ref{fig:introduction}(e). %For this demonstration, the crossbar implementation of SNN, as shown in Fig.\ref{fig:introduction}(c) is considered. 
Fig.\ref{fig:application}(d) illustrates the phenomenon in time domain, where faults happen in some of the synapses, causing no contribution to the output neurons from corresponding inputs and degrade the accuracy. To mitigate that, the 'healthy' astrocyte tripartite synapses can be boosted with the \textit{V}\textsubscript{BG} to recover the output and restore the accuracy. To test the self-repair capabilities on real-world data, we train and test the network on the MNIST handwritten digit recognition dataset \cite{lecun2010mnist}. Details regarding the network and simulation are in the Supplementary section. We obtain a baseline test accuracy of $88.18\%$ on the MNIST test set. Fig. \ref{fig:application}(g) shows the pristine learnt weights. Note, the accuracy of the network can be increased even further by changing the total number of output neurons \cite{diehl2015unsupervised}. Here, we are mainly concerned about the hardware’s self-repair capabilities and thus keep the network size relatively small to reduce the total simulation times. After the initial training, we introduce stuck-at-zero faults (i.e., short-circuits) to the learnt weight patterns (Fig. \ref{fig:application}(h)). The network accuracy drops significantly as the percentage of faults increases as indicated by Fig. \ref{fig:application}(e) and Table \ref{tab:fault_injection}.



To recuperate the accuracy back, we want to employ the astrocyte-like repair mechanism to our “healthy” synapses (Fig. \ref{fig:application}(g-i)). Previous studies on astrocyte computational models realize self-repair by retraining the network with faults in place with an additional astrocytic self-repair scaling factor in the learning rule. This factor dynamically encodes the degree by which the neuron firing rate deviates from the original firing frequency, thus ensuring a similar firing activity after retraining \cite{han2023astromorphic, rastogi2021self}. Obviously, this does not map directly to device dynamics and thus, implementing it on-chip at each cross-point requires significant complexity in the peripherals. Propitiously, the back-gate allows us a much simpler way to implement the factor, while preserving the advantage of using the original device dynamics as shown in eq. \ref{Eq_FeFET_STDP}. By boosting the conductance with the back-gate voltage, $V_{BG}$, the network sees the effective weight, $W_{eff}$ in lieu of the originally programmed post-synaptic weights, $W_{post}$ and modulates the incoming spikes. We can write:\\
\vspace{-7mm}
\begin{equation}
    \label{Eq_I_neuron_self}
    W_{eff} = k*W_{post}
\end{equation}
\vspace{-10mm}

\noindent Here, $k$ is a function of the applied back gate voltage to each column and is henceforth referred as the degree of self-repair. The degree of self-repair needed for each column of weights is adapted as the network is retrained. Further details of the self-repair functionality can be found in the Supplementary Section 'Self-repair Mechanism of the Network'. Table \ref{tab:fault_injection} shows that our self-repair scheme can greatly recover its lost accuracy. Effectiveness of the self-repair process becomes obvious as the number of faults in the network increases. Modifying the weights without having such a back-gate control can not only result in no recovery but in some cases can worsen the network performance after the retraining phase (Table \ref{tab:fault_injection}) – further indicating the efficacy of the back-gate voltage.

% In this study, the network on the MNIST handwritten digit recognition dataset \cite{lecun2010mnist} is trained and tested using the PyTorch based BindsNet framework \cite{hazan2018bindsnet}. A baseline neural network with 784 input neurons and 225 output neurons is trained in an unsupervised manner using Spike-timing dependent plasticity (STDP) learning \cite{bi2001synaptic} and a test accuracy of 83.96\% is obtained. \textcolor{red}{Supplementary table 1} lists the training network parameters. Note that the accuracy of the network can be increased by increasing the total number of output neurons (6400 neurons yield $>$95\% accuracy \cite{diehl2015unsupervised}). The network size is kept small to reduce the total simulation time. After training, stuck-at-zero faults (shorted) to the learnt weight pattern are introduced. The network accuracy drops significantly as the percentage of faults is increased, as shown in Fig.\ref{fig:application}(e). The astrocyte-like repair mechanism can be introduced to the “healthy” synapses by ramping up the corresponding column \textit{V}\textsubscript{BG}. Previous studies on astrocyte computational models have revealed that the amount of weight boost required for self-repair is dependent on the initial weights of the “healthy” synapses \cite{rastogi2021self}. The astrocytic network regularizes the weights connected to a neuron in such a way that the sum of the total weights approximates that of the network without faults – thus keeping the firing rate consistent \cite{han2023astromorphic}. For the crossbar self-repair scenario, this translates as the applied \textit{V}\textsubscript{BG} to each column being proportional to the ratio of the total sum of weights prior to fault (which can be obtained from software) and the total sum of weights after faults are introduced (i.e., the network is embedded in hardware). The sum of weights for a particular neuron/synaptic column can be obtained by activating all the synapses in the columns. It is discovered that after boosting the conductances, the network is able to greatly recover its lost accuracy, as shown in Fig.\ref{fig:application}(e). Additionally, the network’s inference accuracy is not sensitive to variation in \textit{V}\textsubscript{BG}, as shown in Fig.\ref{fig:application}(f), thus indicating great tolerance. \textcolor{red}{Abhronil, can you explain Fig.4(g)-(i)}

\begin{figurehere}
   \centering
    \includegraphics[width=0.95\textwidth]{figures/Fig4_v1.pdf}
    \caption{\textit{\textbf{Working principles of dual-port FeFET as astrocyte.} Potential applications of memory encryption techniques: (a) To prevent from Stolen DIMM attacks, (b) To ensure AI privacy, and (c) To implement in secure encrypted virtualization (SEV) (d) Without protection, NVMs become vulnerable after power down. (e) NVMs with AES-embedded can be protected after power down but with high encryption overheads. (f) With the proposed encryption scheme, NVMs can be protected after power down with minimal penalty.}}
    \label{fig:application}
\end{figurehere}


As an another example of the application of astrocyte is to implement \textcolor{blue}{a model of dragonfly prey-interception circuitry \cite{chance2020interception}, as illustrated in Fig.\ref{fig:application}(j). Visual information from the eye (illustrated in yellow in Fig.\ref{fig:application}(k)) is modeled as the responses of an array of neurons $f(x)$, where $f_i(x)$ is the response of neuron $i$ to $x$, the position of the prey's image on the dragonfly's eye. Similarly, $g(y)$ indicates an array of proprioceptive inputs for which $g_j(y)$ is the response of neuron $j$ encoding the dragonfly's head at position $y$ relative to the dragonfly's body. These two inputs, $f(x)$ and $g(y)$ are mapped into the drain input and the back gate input, respectively (see Fig.\ref{fig:application}(k)).  As a result, the output of each FeFET device will be proportional to the product of the two inputs, $f_i(x)g_j(y)$, such that all possible combinations of visual and proprioceptive inputs are represented in the array of FeFET devices.  While the visual input is in eye-coordinates (relative to the reference frame of the eye), this configuration of input combinations may be thought of as forming a set of basis functions \cite{pouget1997spatial,pouget2000computational} from which motor outputs may be calculated for alternate frames of reference (e.g., body-coordinates). This sensorimotor transformation is achieved by summing linear combinations of the basis functions, or FeFET outputs. In the dragonfly application, the turns required for interception are represented in the responses of the motor neuron population (not drawn). The response of an individual motor neuron, $k$, is proportional to $\sum_{i,j}W_{ijk}f_i(x)g_j(y)$. Fig.\ref{fig:application}(i) illustrates an example trajectory (green symbols) of the dragonfly model from \cite{chance2020interception} intercepting a moving prey (red symbols). For simplicity, the model and prey are constrained to move only within a two-dimensional plane, significantly decreasing the size of the model.  The purple symbols are the trajectory of an analogous model with $g(y)$ ([0,1] in \cite{chance2020interception} mapped to the slope values given in Fig.\ref{fig:synapse}(g). This mapping introduces an offset into the values of $g$, resulting in different behavior of the FeFET-based dragonfly simulation. This offset can be corrected by introducing additional steps into the turn decoding algorithm (not shown).    }     
%\textcolor{blue}{The visual input $f(x)$ and the proprioceptive info $g(y)$ can be mapped into the drain input and the back gate input, respectively, as shown in . In this way, the output will be proportional to the product of the two. \textcolor{blue}{Suma and Frances, can you write this section? Explain how the astrocyte is used to map the model? Explain the experimental setup, how to interpret Fig.4(l). And also, the response is f(x)*g(y) in the proposal. Do you really need the weight here? The Fig.4(k) implements the f(x)*g(y)*Wij}.

\textcolor{magenta}{In addition to self-repair, the back-gate control enables us to implement homeostasis in the crossbar array itself by controlling the effective conductance of an entire column of synaptic devices. In SNNs, homeostasis is essential for learning across all neurons, as it ensures neurons that have fired require a greater input than before to fire again. Without it, only a few neurons dominate, and the network is not able to learn the desired patterns. As illustrated in Fig.\ref{fig:homeostasis}(a), homeostasis is generally enabled in neural networks by increasing the threshold required for a neuron to spike after it fires. In hardware implementation, such regularization is supplemented on top of the neuronal circuitry – adding sizable overhead \cite{rajendran2012specifications, indiveri2003low}, as shown in Fig.\ref{fig:homeostasis}(b). The back-gate control of the DG-FeFET affords us a much more elegant solution (Fig. 4(c)). The back-gate voltage can effectively modulate the output of the crossbar going to the neuron devices as the output is a dot product of the input voltage and device conductances. Thus, by ramping down the back-gate potential of a particular column whenever the neuron associated with it fires, we can achieve homeostasis. We substantiate our claim by integrating these synaptic dynamics in an SNN implementation. We train a network with a similar architecture as before on the MNIST dataset. As the training will take place in our FeFET devices, we utilize a weight-dependent learning rule for the STDP [12]. After 1 epoch of training, we find that the network with back-gate modulation is able to induce homeostasis (Fig. 4(d)), attaining an accuracy of 82.14\% over the test set – on par with networks of similar size [13, 14].} \textcolor{green}{Abhronil, we need to finalize this paragraph and the supplementary so that we do not duplicate.}



==> sections/Introduction.tex <==
\section*{\textcolor{sared}{\large Introduction}}

% [OUTLINE: 1. NVM -> security: NVM-targeted attacks; 2. memory encryption techniques--AES; 3. existing problems-latency; 4. our design-directly encrpt memory itself+low overhead; 5. applications]

Current neuromorphic computing systems are synapse and neuron centric. Inputs from the pre-synaptic neurons are weighted and then integrated in post-synaptic neurons to generate outgoing spikes. This model, however, is not completely bio plausible. In fact, most synapses are tripartite – having a third terminal from astrocytes, a type of glial cell. Although glial cells constitute $\sim50\%$ of all human brain cells \cite{moller2007glial}, their inability to generate electrical impulses led many to regard them as mere supportive structures of the brain for a long time. Recent discoveries, however, suggest they not only work as sensing and communication mediums for various brain regions but also play an active role in regulating spiking behavior across multitudes of neurons -- underlying various brain functionalities \cite{allen2009glia, kuga2011large}. From memory formation and learning to self-repair and neural phase synchrony, contemporary computational analyses have revealed the efficacy of including astrocytic components, i.e., tripartite synapses, to established spiking neural network platforms \cite{han2023astromorphic, rastogi2021self, garg2021emulation}. Fig.\ref{fig:introduction}(a) shows the working principle of a tripartite synapse. Neuromodulators from astrocytes change the transmission probability (PR) of the neurotransmitters from the pre-synaptic neuron to the post-synaptic neuron, thus modulating the effective connection strength of the synapse \cite{perea2007astrocytes}. 
% \textcolor{red}{
% Abhronil, can you say more on the astrocytes and its importance for neuromorphic computing? Right now, it is not developed in a lot of details.
% }


\begin{figurehere}
   \centering
    \includegraphics[scale=1,width=\textwidth]{figures/Fig1.pdf}
    \caption{\textit{\textbf{Motivation and potential applications.} Potential applications of memory encryption techniques: (a) To prevent from Stolen DIMM attacks, (b) To ensure AI privacy, and (c) To implement in secure encrypted virtualization (SEV) (d) Without protection, NVMs become vulnerable after power down. (e) NVMs with AES-embedded can be protected after power down but with high encryption overheads. (f) With the proposed encryption scheme, NVMs can be protected after power down with minimal penalty. \textcolor{blue}{panel d and associated caption need to be fixed - purple layer should be relabeled as "basis functions" or "sensorimotor layer", and/or an output layer needs to be added (I don't think labeling the purple layer as "response" is correct with the current text - Frances) }}}
    \label{fig:introduction}
\end{figurehere}

Given its significance, it calls for efficient hardware implementation to further accelerate the deployment of intelligent neuromorphic devices. Efforts to realize astrocytic functionality in Complementary Metal Oxide Semiconductor (CMOS) hardware thus far has relied on analog circuits \cite{irizarry2013cmos, irizarry2015astrocyte, lee2016cmos} or low complexity FPGAs \cite{karimi2018neuromorphic, nazari2015digital}. Besides being bulky, the focus for these approaches has generally been emulation of neuro-glia computational models with high-precision, rather than computation. Likewise, advances in emerging post-CMOS technologies to implement compact neuromorphic devices \cite{wang2018experimental, saha2021intrinsic} have largely ignored any abstraction of astrocytes. A compact and efficient realization of the astrocyte still remains missing. 
%\textcolor{red}{Abhronil, please say something about the existing implementation using CMOS. What is its challenge}. 
Given these challenges, in this work, we propose a novel single transistor solution, i.e., double gate ferroelectric field effect transistor (DG-FeFET), that can emulate the functionalities of astrocyte. Fig.\ref{fig:introduction}(a) shows a fully-depleted silicon-on-insulator (FDSOI) FeFET, that intrinsically realizes a DG-FeFET. On the top, the ferroelectric thin film is integrated with the top gate (TG) such that the nonvolatile polarization states can store the conventional synapse weight, as have been widely studied in \cite{jerry2017ferroelectric, yu2021ferroelectric}. Beyond the simple synapse function, the FDSOI FeFET also have a back gate (BG) and a non-ferroelectric insulator, i.e., buried oxide (BOX), that also controls the channel current \cite{jiang2022asymmetric, mulaosmanovic2021ferroelectric, zhao2023powering, zhao2024paving}. Due to the thin Si channel, the TG and BG both control the channel and are electrically coupled. Therefore, the synapse weight can be temporarily modulated via the BG, on top of the nonvolatile weight set by the polarization, akin to the astromorphic modulation in the biological astrocyte. In this way, a single transistor with four terminals can realize a compact astrocyte tripartite synapse. Note that this design can also be applicable for other transistor memory, such as charge trap flash. But the superior energy efficiency of ferroelectric HfO\textsubscript{2} based FeFET, its excellent scalability, and CMOS-compatibility \cite{mulaosmanovic2021ferroelectricre} make it a prime candidate for this application. Also with the capability of realizing ferroelectricity in HfO\textsubscript{2} at the back-end-of-line (BEOL) compatible thermal budget \cite{aabrar2022beol, datta2024amorphous}, it is also possible to integrate monolithically 3D integrated DG-FeFET, thus further enhancing the astrocyte synapse density.   

%look at a double gate ferroelectric device (DG-FeFET) that can mimic the functionality of tripartite synapse with the back-gate voltage as our astrocytic control mechanism. We explore the impact of the DG-FeFET devices as synapses in crossbar arrays implementing spiking neural networks (SNNs) – enabling the functionality of homeostasis and self-repair in hardware without incurring additional peripheral cost.
With such a DG-FeFET cell, it then allows a straightforward mapping of the astrocyte in spiking neural networks (SNN) to an FeFET array. Fig.\ref{fig:introduction}(b) illustrates a classical two-layer SNN with pre-synaptic input neurons and post-synaptic output neurons, but with astrocyte tripartite synapses connected between them. 
% \textcolor{red}{Abhronil, in the real implementation, do we need to tune each synapse using BG individually? Or we can share the BG per column. The latter case, shown in Fig.1(c) correspond to that each output neuron has one shared VBG. -- No, each synapse does not need to be tuned individually. Yes, we can share the BG per column. Fig.1(c) shows this correctly. device. Text:} 
The back gates of all the synapses along the columns are connected. This not only greatly simplifies the complexity of implementation but also mimics the similar type of non-local modulation seen in real astrocytes. Input voltages are fed along the pre-synaptic terminals and are modulated by synapse conductance before being summed up at the post-synaptic terminals. %\textcolor{red}{Additional access transistors are present to ensure proper operation. For further details of how such crossbar systems work, readers are referred to \cite{saha2021intrinsic}.} \textcolor{cyan}{We do not necessarily need access transistor.} 
In one array design, as shown in Fig.\ref{fig:introduction}(c), the astromorphic modulation is mapped into a column-wise BG input and the pre-synaptic and post-synaptic neurons are mapped as input and output of the FeFET pseudo-crossbar array, respectively. Though the single transistor array can be successfully operated \cite{jiang2022feasibility, xiao2022write}, if needed, an access transistor can be added for each FeFET for better management of write disturb \cite{saha2021intrinsic}. In this design, to save the space for the BG wire routing, the granularity of BG control is defined per post-synaptic neuron. In this way, the pseudo-crossbar array can perform the intended matrix-vector multiplication while the synapses can be temporarily modulated via the exerted BG biases. In FDSOI FeFET, the BG is realized with a p-well contact. Therefore, the implementation of the column-wise BG can be realized through column-wise p-well contact and necessary isolation between neighboring p-wells. For the BEOL DG-FeFET implementation, it is possible to directly adopt a metal BG, such that the density of integration is higher than the FDSOI FeFET.  


Such a kernel with an array of astrocyte tripartite synapses, if available, could enable many important applications, such as efficient hardware emulation of biological models such as a dragonfly prey interception model as shown in Fig.\ref{fig:introduction}(d), SNN self-repair \cite{navarrete2010endocannabinoids} as shown in Fig.\ref{fig:introduction}(e), and homeostasis, as explained in Fig.\ref{fig:homeostasis}. 
\textcolor{blue}{For successful prey interception, a dragonfly must transform visual information in "eye" or "camera" coordinates into motor commands expressed in "body" coordinates. To perform this transformation, the dragonfly prey interception model relies upon a set of basis functions encoded by a layer of gain-modulated units (purple in Fig.\ref{fig:introduction}d). These units combine visual information with dragonfly head position information via a gain control mechanism supported by the astrocyte tripartite synapse.} For the self-repair application, 
the astrocyte tripartite synapse has been attributed with performing self-repair in the brain of damaged synapses \cite{navarrete2010endocannabinoids}. From computational neuroscience modeling \cite{rastogi2021self}, whenever faults are introduced to a network, i.e., by changing their propagation probability to zero, as shown in Fig.\ref{fig:introduction}(e), the astrocyte mediated system increases the propagation probability of healthy synapses to ensure recovery of the firing rate of the post-synaptic neuron and repairing the impact of fault introduction. \textcolor{magenta}{Tripartite synapse also offers a new method for homeostasis, crucial for neuron activity regulation. In conventional approach, the firing threshold for the output neuron is increased temporarily, as illustrated in Fig.\ref{fig:homeostasis}(a). However, hardware implementation of flexible threshold tuning is nontrivial. On the other hand, the tripartite synapse can circumvent the complexity by adjusting synapse strength through reducing the back gate bias without changing the output neuron, as shown in Fig.\ref{fig:homeostasis}(e).} \textcolor{cyan}{Abhronil, please check.}

%Neuromorphic hardware for implementing spiking neural networks (SNNs) has gained interest by applying nonvolatile memory (NVM) for synaptic weight cells. However, most developed synapses lack the third terminal for additional weight modulation, only offering programmable conductance between pre- and post- neurons. In our study, we investigate a double-gate FeFET (DG-FeFET) that emulates a tripartite synapse, using back-gate voltage as an astrocytic control mechanism (Fig.2(c)). We analyze its impact on crossbar arrays implementing SNNs, enabling hardware homeostasis and self-repair without extra peripheral costs.


\subsection*{Modeling Dendrites using DG-FEFETs}
\textcolor{green}{Dendrites are frequently overlooked in models of biological neurons, often being simplified to mere wires. However, emerging research suggests that they play a crucial role in a variety of complex functions within a single neuron, including non-linear filtering, spatio-temporal integration, and gain modulation, etc~\cite{poirazi2020illuminating}.}

\textcolor{green}{Bio-inspired artificial neurons, such as the perceptron \cite{mcculloch1943logical,rosenblatt1958perceptron}, are commonly described as performing a weighted sum of their inputs, $\sum_{i}W_{i}I_{i}(t)$. Compared to the fixed input weights for the perceptron model, we consider a biologically-inspired gain modulation mechanism by which input weights may be modified in a continuous or streaming manner.
    While mathematically equivalent to modifying synaptic input weights, this mechanism can also be thought of as modifying the gain of individual branches of dendrites, or sets of inputs and their weights. The result is a multiplicative scaling of the response curve (as seen in Figure --). This allows for \textit{dynamic reconfiguration} of weights as opposed to fixed synaptic weights for a static change.  ``Gain fields'' \cite{andersen1983influence}, where information encoded in different coordinate systems (e.g., eye-centered vs body-centered reference frames) are multiplicatively combined through gain modulation of a neuron's responses, have been reported in a wide range of brain areas (see \cite{salinas2000gain} for a review) and are thought to have critical roles in spatial transformations \cite{pouget1997spatial, pouget2000computational, salinas2001coordinate} performed in the brain.}

\textcolor{green}{Chance and Cardwell have previously proposed shunting inhibition, a type of synaptic input that ``shunts'' the dendritic resistance, thereby changing the overall gain of the neuron~\cite{chance2023shunting,cardwell2023dendritic}, as an effective approach to dynamic gain modulation. In this work, we utilize a DG-FeFET-based dendrite that supports multiplicative gain modulation. We further demonstrate this FEFET dendrite in a dragonfly interception circuit model demonstrated by Chance. We have simplified the model by constraining both the dragonfly and its prey to two-dimensional movement rather than three-dimensional. This adjustment considerably reduced the model's complexity, facilitating its implementation in hardware. Our primary objective is to demonstrate that FeFET-based dendrites can effectively replace the layer of multiplicative neurons in the original model, offering improved performance efficiency. The visual input $x$ encodes the position of the prey on the dragonfly's eye and the second population denotes the ``desired position'' of the prey for the correct turn the dragonfly must make to intercept it. The hidden layer referred to as sensorimotor}
neurons each combine input from one visual input
and the desired-position input j by multiplying the two signals, $I(x)G(y)$. 











==> sections/Overview.tex <==
\section*{\textcolor{sared}{\large Double-gate FeFET as astrocyte tripartite synapse}}

Next, the origin of the capability of DG-FeFET to function as an astrocyte tripartite synapse is clarified. In a DG-FeFET, such as the FDSOI FeFET, the top ferroelectric gate can be used to program the synaptic weight by exploiting partial polarization switching to access the analog states and the bottom BG can act as astrocyte to modulate the channel conductance, thus realizing a compact astrocyte tripartite synapse. To understand how the BG bias, \textit{V}\textsubscript{BG}, modulates the DG-FeFET, it is necessary to look at the electrostatics and transport properties. Fig.\ref{fig:device_principle}(a) and (b) show the gate stack and equivalent circuit symbols, respectively. It has been well established that the top gate device threshold voltage (\textit{V}\textsubscript{TH}) can be linearly shifted by the \textit{V}\textsubscript{BG} \cite{mulaosmanovic2021ferroelectric, lim1983threshold}, with a linear coefficient $\gamma$\textsubscript{TG}, which is defined as
\begin{equation} \label{Eq.1}
    \gamma_{TG} = \cfrac{\cfrac{C_{CH}*C_{BGOX}}{C_{CH}+C_{BGOX}}}{C_{TGOX}}
\end{equation}
\noindent where the \textit{C}\textsubscript{TGOX}, \textit{C}\textsubscript{CH}, and \textit{C}\textsubscript{BGOX} are the top gate oxide capacitance, the channel capacitance, and the back gate oxide capacitance, respectively, as defined in Fig.\ref{fig:device_principle}(a) and (b). With this linear dependence, the channel conductance, \textit{G}\textsubscript{DS}, sensed at the top gate at a given \textit{V}\textsubscript{BG} can be related with the \textit{G}\textsubscript{DS} at \textit{V}\textsubscript{BG}=0V, as explained in Fig.\ref{fig:device_principle}(c). The relationship can be expressed as
\begin{equation} \label{Eq.2}
    G_{DS}(V_{BG}) = \frac{\mu_n(V_{BG})}{\mu_n(V_{BG}=0)}G_{DS}(V_{BG}=0)+\gamma_{TG}\cdot\mu_n(V_{BG})\cdot C_{TGOX} \cdot V_{BG}
\end{equation}
where the $\mu_n(V_{BG})$ and $\mu_n(V_{BG}=0)$ are the electron mobility at a nonzero and zero \textit{V}\textsubscript{BG}, respectively. One interesting property of FDSOI transistor is that the electron mobility increases with the \textit{V}\textsubscript{BG}. This is because at a higher \textit{V}\textsubscript{BG}, the carrier centroid in the channel will move away from the interface between the top gate dielectric and channel, thus reducing the Coulomb scattering and surface roughness scattering \cite{nier2013multi, al2022impact, han2022back}. Within a reasonable range of \textit{V}\textsubscript{BG}, the mobility can be approximated as a linear function of \textit{V}\textsubscript{BG} \cite{nier2013multi}. Therefore, the \textit{G}\textsubscript{DS} at a nonzero \textit{V}\textsubscript{BG} will be linearly dependent on the \textit{G}\textsubscript{DS}(\textit{V}\textsubscript{BG}=0) with a slope proportional to \textit{V}\textsubscript{BG}. Fig.\ref{fig:device_principle}(d) and (e) illustrates a qualitative picture of \textit{G}\textsubscript{DS} sensed at different \textit{V}\textsubscript{BG}s during synaptic potentiation and depression and the corresponding \textit{G}\textsubscript{DS} dependence on the \textit{G}\textsubscript{DS}(\textit{V}\textsubscript{BG}=0). This dependence will be experimentally validated in the following paragraphs.

\begin{figurehere}
   \centering
    \includegraphics[width=1\textwidth]{figures/Fig2_v2.pdf}
    \caption{\textit{\textbf{Working principles of dual-port FeFET as astrocyte.} Potential applications of memory encryption techniques: (a) To prevent from Stolen DIMM attacks, (b) To ensure AI privacy, and (c) To implement in secure encrypted virtualization (SEV) (d) Without protection, NVMs become vulnerable after power down. (e) NVMs with AES-embedded can be protected after power down but with high encryption overheads. (f) With the proposed encryption scheme, NVMs can be protected after power down with minimal penalty.}}
    \label{fig:device_principle}
\end{figurehere}

%Next it is important to understand how the astrocyte terminal controls the synapse. To do that, it is necessary to examine the double gate operation principles and conduct experimental validation. For that, industrial FDSOI FeFETs integrated 22nm FDSOI technology platform is adopted for experimental testing (Fig.3(a) and (b)) featuring an around 10nm doped HfO2 [7].

In this way, it can be seen that the \textit{G}\textsubscript{DS} will be proportional to the product of the \textit{G}\textsubscript{DS}(\textit{V}\textsubscript{BG}=0) and the \textit{V}\textsubscript{BG}. If the nonvolatile weight in the astrocyte tripartite synapse is mapped to \textit{G}\textsubscript{DS}(\textit{V}\textsubscript{BG}=0) and the transient astromorphic modulation input is mapped to \textit{V}\textsubscript{BG}, the simple single transistor DG-FeFET realizes the astrocyte tripartite synapse. Next experimental validations are performed to confirm the intended functionalities. In this work, the FDSOI FeFET, shown in Fig.\ref{fig:device_principle}(f), is adopted given that it intrinsically has a double gate structure. For that, industrial FDSOI FeFETs integrated 22nm FDSOI technology platform is adopted for experimental testing \cite{dunkel2017fefet}. The device transmission electron microscropy cross section is shown in Fig.\ref{fig:device_principle}(g). The device
features a 10 nm thick atomic layer deposited doped HfO\textsubscript{2} as the ferroelectric. Detailed process information is described elsewhere \cite{dunkel2017fefet}. Fig.\ref{fig:device_principle}(h) and (i) show the \textit{I}\textsubscript{D}-\textit{V}\textsubscript{G} characteristics and corresponding \textit{V}\textsubscript{TH} measured at the top gate, respectively, for the low-\textit{V}\textsubscript{TH} and high-\textit{V}\textsubscript{TH} states sensed at different \textit{V}\textsubscript{BG}s. It clearly shows that \textit{V}\textsubscript{TH} for both states decreases linearly with the \textit{V}\textsubscript{BG} due to electrostatic coupling. The memory window (MW), however, remains constant with the \textit{V}\textsubscript{BG}. Similarly, Fig.\ref{fig:device_principle}(j) and (k) show the \textit{I}\textsubscript{D}-\textit{V}\textsubscript{G} characteristics sensed at the bottom gate and corresponding \textit{V}\textsubscript{TH} at different front gate biases. It also shows that the back gate \textit{V}\textsubscript{TH} is linearly dependent on the front gate bias. An interesting fact is that the memory window sensed at the back gate is much higher than that sensed at the front gate, which is due to the thick gate dielectric at the back gate. This window amplification, however, can not increase the number of available states as it amplifies both the window and the variation of the front gate \cite{chatterjee2022comprehensive}.  


\begin{figurehere}
   \centering
    \includegraphics[width=1\textwidth]{figures/Fig3_v1.pdf}
    \caption{\textit{\textbf{Working principles of dual-port FeFET as astrocyte.} Potential applications of memory encryption techniques: (a) To prevent from Stolen DIMM attacks, (b) To ensure AI privacy, and (c) To implement in secure encrypted virtualization (SEV) (d) Without protection, NVMs become vulnerable after power down. (e) NVMs with AES-embedded can be protected after power down but with high encryption overheads. (f) With the proposed encryption scheme, NVMs can be protected after power down with minimal penalty.}}
    \label{fig:synapse}
\end{figurehere}

Next, the astrocyte tripartite synapse emulated using the DG-FeFET is characterized. Following standard practice for artificial synapses, three pulse schemes are applied: identical pulse trains, pulse width modulation, and pulse amplitude modulation, as illustrated in Fig.~\ref{fig:synapse}(a), (b), and (c), respectively. The corresponding gate pulse amplitudes and widths are presented for each scheme. During synaptic potentiation and depression, the source, drain, and back gate are grounded. Conductance measurements are performed by sweeping the \textit{I}\textsubscript{D}-\textit{V}\textsubscript{G} characteristics on the top gate under different \textit{V}\textsubscript{BG} conditions. The corresponding conductance tuning characteristics resemble those reported on FeFET that the identical pulse scheme yields the worst tuning characteristics \cite{jerry2017ferroelectric}, where it exhibits very limited number of states. The number of intermediate states can be increased with varying pulse widths as more domains can participate in the switching, but there is a strong asymmetry and nonlinearity between potentiation and depression. In contrast, the pulse amplitude modulation exhibits the best characteristics, where it shows an almost linear and symmetric potentiation and depression.   
Aside from confirming the well-established synaptic behavior in FeFETs, these results also validate that the synaptic weight can be modulated by the \textit{V}\textsubscript{BG}, where the higher the \textit{V}\textsubscript{BG}, the higher the conductance, thus showing the desired astrocyte function. Such weight programming and astrocyte modulation are reproducible, as seen in 10 times repeated measurement of the pulse width modulation scheme shown in Fig.\ref{fig:synapse}(d) and the pulse amplitude modulation scheme shown in Fig.\ref{fig:synapse}(e). 


If plotting the measured conductance at different \textit{V}\textsubscript{BG}s with respect to that at \textit{V}\textsubscript{BG}=0V, as shown in Fig.\ref{fig:synapse}(f), a linear dependence is presented, consistent with Eq.\ref{Eq.2}. In addition, the extracted slope of the linear fitting, as shown in Fig.\ref{fig:synapse}(g), is also linearly dependent on the \textit{V}\textsubscript{BG}, again confirming the theoretical analysis shown in Eq.\ref{Eq.2}. It also indicates that within a resonable range of \textit{V}\textsubscript{BG}, the mobility is linearly increasing with the \textit{V}\textsubscript{BG}. Therefore, these results establish that the device conductance is a product between the \textit{V}\textsubscript{BG} and the nonvolatile conductance at \textit{V}\textsubscript{BG}=0V, which emulates a function of astrocyte tripartite synapse. The weight modulation is also highly robust and reproducible, therefore validating the astrocyte functionality. Next the state stability is measured. First, the switching dynamics of the FDSOI FeFET is characterized, as presented in supplementary Fig.\ref{fig:dynamics}. It shows that there is a large basin around 0V, indicating it is difficult to flip the polarization states around 0V, thus good for retention. This has been verified by measuring the retention for the intermediate states at room temperature. As shown in Fig.\ref{fig:synapse}(h), there is negligible degradation for all the states, showing the nonvolatility. Therefore, all the aformentioned combined theoretical and experimental analysis validate the capability of DG-FeFET in realizing the astrocyte tripartite synapse.



==> sections/coverletter.tex <==


\newpage

\noindent
Dear Editors and Reviewers,

\noindent
Please find the enclosed manuscript entitled \textbf{``A Bio-inspired Asymmetric Double-Gate Ferroelectric FET for Emulating Astrocyte and Dendrite Dynamics in Neuromorphic Systems"}, 
which we wish to be considered for publication in Nature Nanotechnology. We believe our work addresses the challenge of advancing neuromorphic computing paradigms beyond conventional neuron–synapse models by introducing for the first time a bio-inspired compact hardware analogue that can mimic astrocytic and dendritic dynamics observed in biological neural networks -- paving the path forward for more efficient, complex, versatile and adaptive neuromorphic systems.    

\noindent
Conventional neuromorphic architectures have predominantly focused on emulating the behavior of neurons and synapses. However, a growing body of research indicates that components like dendrites and astrocytes — once regarded merely as support structures — play crucial roles in dynamically modulating neural processing and contributing ultimately to the emergence of the brain’s remarkable intelligence. In order to translate the advantages of these biological mechanisms to neuromorphic hardware, we propose an asymmetric Double Gate Ferroelectric FET (DG-FeFET) design featuring a ferroelectric top gate for traditional synaptic weight programming and a non-ferroelectric back gate for dynamic astrocytic/dendritic gain modulation. By leveraging a fully-depleted silicon-on-insulator (FDSOI) platform, we fabricate and verify through theoretical and experimental studies that the back gate can linearly tune the channel’s conductance in conjunction with the partial polarization switching of the ferroelectric layer through the top gate. We show that this configuration replicates an astrocyte tripartite synapse and/or a dendritic arbor with spines and enables exciting applications such as self-repair in faulty neuromorphic hardware (astrocyte-mediated) and specialized computations like coordinate transformations (dendrite-inspired) as seen in biological dragonfly prey-interception neural circuitry.  

\noindent
Our key contributions include: 

\begin{itemize}
    \item \textbf{Novel Asymmetric DG-FeFET Technology:} We present a single device with a dual control mechanism (a ferroelectric top-gate and non-ferroelectric bottom gate) that can imitate astrocyte-regulated tripartite synapses and dendritic gain modulation. To the best of our knowledge, this is the first such reconfigurable hardware demonstration of higher-order neuronal functionalities in neuromorphic systems. Moreover, the transistor-like operation and footprint makes the technology incredibly efficient and easily-integrable in crossbar-based neuromorphic accelerators.
    % \textcolor{blue}{Revise}

    \item \textbf{Emulating Biologically Inspired Astrocytic and Dendritic Dynamics:} By manipulating the back gate potential, we can achieve dynamic modulation and adaptive behavior similar to biological astrocytes and dendrites in neuromorphic hardware. Our device captures crucial neural processing characteristics beyond basic neuron–synapse dynamics.

    \item \textbf{Experimental Validation:} Using an FDSOI FeFET platform, we empirically validate the proposed device’s linear gain control and synaptic behavior, demonstrating robust programmability and reliable performance under various operating conditions.

    \item \textbf{Advanced Neuromorphic Applications} We showcase practical examples such as autonomous hardware self-repair (facilitated by astrocyte-like adaptation) and neuron–dendrite computational tasks (e.g., dragonfly-inspired coordinate transformations for prey interception), underscoring the device’s versatility for diverse neuromorphic solutions.

\end{itemize} 

\noindent
By integrating astrocytes and dendrites into neuromorphic hardware, our DG-FeFET design significantly expands the functional repertoire of current AI accelerators. We fervently believe this work addresses key limitations of standard neuromorphic architectures and opens new avenues for developing truer “brain-like” systems. that go beyond focusing solely on neurons and synapses.

\noindent
We sincerely appreciate your consideration of our manuscript and look forward to engaging with the reviewers’ thoughtful insights and feedback.

\noindent
Sincerely, \\
Abhronil Sengupta and Kai Ni
